An Algorithm for Context-Free Path Queries over Graph Databases

RDF (Resource Description Framework) is a standard language to represent graph databases. Query languages for RDF databases usually include primitives to support path queries, linking pairs of vertices of the graph that are connected by a path of labels belonging to a given language. Languages such as SPARQL include support for paths defined by regular languages (by means of Regular Expressions). A context-free path query is a path query whose language can be defined by a context-free grammar. Context-free path queries can be used to implement queries such as the "same generation queries", that are not expressible by Regular Expressions. In this paper, we present a novel algorithm for context-free path query processing. We prove the correctness of our approach and show its run-time and memory complexity. We show the viability of our approach by means of a prototype implemented in Go. We run our prototype using the same cases of study as proposed in recent works, comparing our results with another, recently published algorithm. The experiments include both synthetic and real RDF databases. Our algorithm can be seen as a step forward, towards the implementation of more expressive query languages.

==> algs/backup/context-free-relations.tex <==
\mm{inicio}

\begin{definition}[Context-Free Grammar with Nested Production Rules] A \textit{Context-Free Grammar with Nested Production Rules (NCFG)} is a \textit{Context-Free Grammar} $G = \tuple{N, \Sigma, P}$, where: (i) the alphabet $\Sigma$ includes the special terminal symbols \em{``[''} and \em{``]''} (not belonging to the language generated by $G$, and (ii) the set $P$ of production rules  are of the form $\Rule{X}{\alpha}$, where $X \in N$ and $\alpha \in (N \cup \Sigma)^*$ is an arbitrary sequence of terminal and non-terminal symbols that may include nested pairs of \em{``[''} and \em{``]''}.
\hfill$\Box$
\end{definition}

The function computed by our query processing algorithm is defined as follows:

Given $D = \tuple{V, E}$, the graph, augmented with explicit inverted edges; 
a NCFG $G=\tuple{N, T, P}$;
and the query $Q=\subseteq V \times N$, we define the set of answers $$\textit{Answers}(Q) = \set{b \ |\ (a, X) \in Q \ \mathit{and}\ b \in R(a, X)}.$$

The function $R\subseteq V \times N \mapsto 2^V$ is inductively defined on the structure of the right-hand side of the production rules of $G$:

\begin{description}
\item[case $\epsilon$:] For any vertex $a\in V$, we define we define $a \in R(a, \epsilon)$.
Moreover, for any rule $\Rule{X}{\epsilon} \in P$, we define $a \in R(a, X)$.

\item[case $b$:] For any terminal symbol $p \in T - \set{], [}$ and edge $(a,p,b)\in E$, we define $b \in R(a, p)$.

Moreover, for any rule $\Rule{X}{p}$, we define $b \in R(a, X)$.

\item[case nested:] For any vertex $a\in V$, we define $(a, X, a) \in R$ if and only if exists $b\in V$ such that $(a, X, b) \in R$
\end{description}


\mm{fim}

==> algs/backup/get-or-create.tex <==
% \KwIn{$node *Node, label string, G *Grammar$}
% \KwResult{Relation}  
\SetKwProg{function}{function}{}{end}
\function{get\_or\_create$(node,label)$}{ %\ciro{(math-like version)}
    \If{$(node,label) \notin R$}{
        $r := (node, label, \emptyset, \emptyset)$ \label{ln:create-relation} \\
        \If{$label \in \nonterminals$} { % nonterminals
            $r.rules := \set{parse(rhs) ~|~ \Rule{label}{rhs} \in \rules} $ \label{ln:build-rules}
        }\ElseIf{$label \in \terminals$} { % terminals
            $r.answers := \set{b ~|~ (a,label,b) \in D}$ \label{ln:get-answers-from-graph}
        }\Else { %  expressions
            \ciro{$label$ is an expression (delete this clause?)} \\
            $r.rules := \set{parse(label)}$
        }
        R(node,label) := r \label{ln:map-new-relation} % TODO: do not add nil relations 
    }
    \Return R(node, label)
}

% Relation structure
% Node()    string
% Label()   string
% Objects() nodeMap
% rules

==> algs/backup/hellings2015.tex <==
\subsection{Path Results for Context-free Grammar Queries on Graphs~\cite{Hellings2015pathresults}}
The most relevant work, however, to this research is J. Hellings~\cite{Hellings2015pathresults}.
Instead of adding grammar informaiton to the graph, the author proposes to build grammars with information from the graph.
They are the graph-annotated context-free grammars.

The main idea in this approach is to annotate non-terminals in the grammar's production rules with graph vertices, in such a way that those rules produce only valid paths.

An annotated non-terminal has the form $X{[a,b]}$, what means that there exists a path from $a$ to $b$ that can be derivable by $X$.
The algorithm for constructing annotated grammars has some similarities with the one proposed in the author's previous work~\cite{Hellings14}, among them the fact that it only works with grammars in the CNF.
The reader may refer to the paper to get an in-depth explanation on how that algorithm works.

\begin{figure}[h]
\centering
% \includegraphics[width=.5\textwidth]{figures/ex-annot}
\caption{Grafo Exemplo~\cite{Hellings2015pathresults}.}
\label{fig:ex-annot}
\end{figure}

\begin{grammar}
\label{gram:ex-annot}
Define a linguagem $\textit{friendOf}^+$.
\begin{enumerate}
\item $\Rule{S}{\textit{friendOf}}$
\item $\Rule{S}{S~S}$
\end{enumerate}
\end{grammar}

Dado o grafo da \autoref{fig:ex-annot} e a \autoref{gram:ex-annot}, a avaliação da consulta $Q \equiv_{def} S(x,y)$ provoca a criação da seguinte gramática anotada.

\begin{grammar}
Gramática anotada resultado da execução do algoritmo~\cite{Hellings2015pathresults}.
\begin{enumerate}
\item $\Rule{S[Alice,Bob]}{\textit{friendOf}}$ \label{r:ab}
\item $\Rule{S{[Alice,Craig]}}{\textit{friendOf}}$
\item $\Rule{S{[Bob,Dan]}}{\textit{friendOf}}$ \label{r:bd}
\item $\Rule{S{[Craig,Eve]}}{\textit{friendOf}}$
\item $\Rule{S{[Dan,Eve]}}{\textit{friendOf}}$ \label{r:de}
\item $\Rule{S{[Alice,Dan]}}{S{[Alice,Bob]} ~S{[Bob,Dan]}}$ \label{r:abd}
\item $\Rule{S{[Alice,Eve]}}{S{[Alice,Bob]} ~S{[Bob,Eve]}}$ \label{r:abe}
\item $\Rule{S{[Alice,Eve]}}{S{[Alice,Craig]} ~S{[Craig,Eve]}}$ \label{r:ace}
\item $\Rule{S{[Alice,Eve]}}{S{[Alice,Dan]} ~S{[Dan,Eve]}}$ \label{r:ade}
\item $\Rule{S{[Bob,Eve]}}{S{[Bob,Dan]} ~S{[Dan,Eve]}}$ \label{r:bde}
\end{enumerate}
\end{grammar}

Com esta gramática anotada, é possível construir apenas caminhos válidos no grafo. Se quiséssemos, por exemplo, produzir um caminho real entre $Alice$ e $Eve$, poderíamos realizar as seguintes derivações:
\begin{eqnarray*}
\underline{S[Alice,Eve]} &\overset{\ref{r:ade}}{\Rightarrow}&
\underline{S[Alice,Dan]} ~S[Dan,Eve] \\
&\overset{\ref{r:abd}}{\Rightarrow} & \underline{S[Alice,Bob]} ~S[Bob,Dan] ~S[Dan,Eve] \\
&\overset{\ref{r:ab}}{\Rightarrow} & \textit{friendOf} ~\underline{S[Bob,Dan]} ~S[Dan,Eve] \\
&\overset{\ref{r:bd}}{\Rightarrow} &\textit{friendOf} ~\textit{friendOf} ~\underline{S[Dan,Eve]} \\
&\overset{\ref{r:de}}{\Rightarrow} & \textit{friendOf} ~\textit{friendOf} ~\textit{friendOf}
\end{eqnarray*}

The runtime and space complexity of the algorithm are respectively $\bigO(|P'_\epsilon| + |P'_\terminals| + |E| + (|N||V|)^3)$ and $\bigO(|C| + (|N||V|)^3)$, where $P'_\epsilon$ are empty production rules and $P'_\terminals$ are production rules with only one terminal on its right-hand side.

By the end of the paper, the author points out as an open problem whether it is possible to write more efficient algorithms for evaluating queries with specific non-terminal symbol, start and end nodes.

==> algs/backup/main-alg.tex <==
% \KwIn{$D *Graph, G *Grammar, Q []Pair$}
% \KwResult{$V \times E : R$}
\SetKwProg{function}{function}{}{end}
\function{main}{
    \Globals{
        \label{ln:start-globals}
        $D : V \times E \times V$, \\
        $G = (\nonterminals, \terminals, \rules) $, \\
        $Q : V \times \nonterminals $ \\
        % Initialize set of relations R with terminal relations
        $ R : V \times E \mapsto Relation$ \\ %= \set{(s,p) \mapsto \set{o ~|~ (s,p,o) \in D}}$ \\
        % Initialize set of relations R with terminal relations
        % $ O := V \times E : NodeSet$ \\
        $NEW : V $ \label{ln:end-globals} \\
        % $O := \set{ (node,symbol) \mapsto \emptyset ~|~ a \in V \wedge X \in \nonterminals}$ \\
    }
    
    \ForEach{$(node,symbol) \in Q$} {
        \label{ln:start-create-query-relations}
        get\_or\_create(node,symbol)
        \label{ln:end-create-query-relations}
    }
    
    \While{$ NEW \neq \emptyset $}{
        \label{ln:start-main-loop}
        n := pickAndRemove($NEW$) \\
        processNew(n)
        \label{ln:end-main-loop}
    }

    \Return R
}


==> algs/backup/old-example.tex <==
\subsection{Example}
\label{sec:example}
Let us now present an example.
Consider the data graph in Figure~\ref{fig:example-input}.
We want to know what are the reachable vertices starting from $1$ and walking through a path of nested balanced and sequential pairs of $a$'s and $b$'s.
In order to restrict the paths followed by the algorithm to those complying with that constraint, we use Grammar~\ref{gram:unambiguous} (p.~\pageref{gram:unambiguous}), which defines the language $(a^nb^n)^*$.
The input parameters then are the graph $D$, grammar $G_{\ref{gram:unambiguous}}$ and the query $H = \set{(1,S)}$.

\begin{figure}[h]
\centering
\input{fig/example}
\caption{Example graph.}
\label{fig:example-input}
\end{figure}

The algorithm first initializes \I and $D'$.
At line~\ref{l:let-I}, the set of generalized items is initialized as $\I = \set{\Rule{S}{\set{1\u} ~a~ \emptyset ~S~ \emptyset ~b~ \emptyset ~S}, \Rule{S}{\set{1\u}}}$.
The graph $D'$ is just a copy of $D$.
Now that there are unmarked vertices in the positions sets of the elements in \I, the algorithm starts picking them arbitrarily. % non-deterministically.

Let us suppose the algorithm has chosen $x\u = 1\u$ from the item $\Rule{S}{\set{1\u} ~a~ \emptyset ~S~ \emptyset ~b~ \emptyset ~S}$.


\begin{eqnarray*}
I &=& \{ \Rule{S}{\set{1\m} ~a~ \set{3\m,4\m} ~S~ \set{2\m,3\m,4\m} ~b~ \set{3\m,2\m}} \\
&&\ \ \Rule{S}{\set{1\m}}, \\
&&\ \ \Rule{S}{\set{2\m}~a~ \emptyset ~S~ \emptyset ~b~  \emptyset}, \\
&&\ \ \Rule{S}{\set{2\m}}, \\
&&\ \ \Rule{S}{\set{3\m} ~a~ \set{1\m} ~S~ \set{1\m,3\m,4\m} ~b~  \set{4\m}}, \\
&&\ \ \Rule{S}{\set{3\m}}\\
&&\ \ \Rule{S}{\set{4\m} ~a~ \emptyset ~S~ \emptyset ~b~  \emptyset}, \\
&&\ \ \Rule{S}{\set{4\m}} \}
\end{eqnarray*}

\begin{figure}[h]
\centering
\input{fig/result}
\caption{Representation of result graph.}
\label{fig:example-result}
\end{figure}


==> algs/backup/old-explanation.tex <==
The evaluation algorithms compute the transitive closure of relations based on the graph and the grammar's production rules, taking advantage of common prefixes that paths may share.
The basic idea behind this process is similar to what is done by parsers when they use a dot ($\cdotp$) to mark the progress of derivations.
The difference is that instead of a dot, we mark the derivation progress with graph nodes.

Our algorithms maintain a set of relations (see Definition~\ref{def:relation}).
A relation has a unique identifier pair $(node, symbol)$, and a set of $answers$.
It is called a \emph{terminal} or \emph{non-terminal} relation depending on whether $symbol \in \terminals$ or $symbol \in \nonterminals$.
The answers of terminal relations are static, obtained from the graph $D$, as described in Definition~\ref{def:relation}, Base case~\ref{def:relation-bc-terminal}.

The set of $answers$ of a non-terminal relation is computed in an incremental fashion, similar to what is done by parsers during a derivation.
As a parser eats symbols from the input string, it advances a dot in a production rule to keep track of the derivation process.
When the dot reaches the end of the rule, it means that derivation is complete and, for example, a reduction can be applied.
In our approach, a non-terminal relation has a copy of it's symbol's production rules, and we mark the derivation progress with node sets instead of a dot.
As the algorithm ``eats'' edge labels from the graph we make copies of these nodes flow from the start to the end of each rule.
When a node reaches the end of a rule, it becomes part of the relation's answers.
The annotated rules are represented as a list of interleaving node sets and symbols, as shown in Figure~\ref{fig:ex-relations} (the reader may also refer to the implementation in Program~\ref{prog:structs}).

\begin{figure}[h]
    \centering
    
    % \input{fig/ex-relations.tex}
    
    \includegraphics[width=.75\textwidth]{fig/explanation}
    \caption{Illustration of how the algorithm represents \R{a}{S} relations (intermediate step in path the recognition process)}
    \label{fig:ex-relations}
\end{figure}

\begin{program}[h]
    \lstset{basicstyle=\ttfamily, numbers=left, numbersep=5pt, numberstyle=\tiny, stepnumber=1, escapechar=\!, columns=fullflexible, morekeywords={true, false, a, @prefix}}
    \begin{lstlisting}
type Relation struct {
    node      string
    label     string
    answers   (set of nodes)
    rules   []*NodeSet
}

type Symbol struct {
    subjNodeSet *NodeSet
    predicate   string
    objNodeSet  *NodeSet
}

type NodeSet struct {
    nodes    (set of old nodes)
    new      (set of new nodes)
    prev     *Symbol
    next     *Symbol
    relation *Relation
}
    \end{lstlisting}
\caption{Data structures used in the implementation.}
    \label{prog:structs}
\end{program}


The idea described above is implemented with three algorithms.
Algorithm~\ref{alg:main} is the main control function, responsible for declaring global variables (lines~\ref{ln:start-globals}-\ref{ln:end-globals}), initializing relations (lines~\ref{ln:start-create-query-relations}-\ref{ln:end-create-query-relations}) and running until there is no new information to be processed (lines~\ref{ln:start-main-loop}-\ref{ln:end-main-loop}).
To keep track of what information is new, the node sets may have \emph{new} (unprocessed) and \emph{old} (processed). elements.Algorithm~\ref{alg:get-or-create} is a function that accesses relations and Algorithm~\ref{alg:process-new} is the procedure for processing new information.
Their behavior is explained next.

\begin{algorithm}[h]
    \input{algs/backup/main-alg}
	\caption{Main control function.}
	\label{alg:main}
\end{algorithm}

Algorithm~\ref{alg:get-or-create} provides access to relations given their identifier pair.
If a relation does not exist, it is created (line~\ref{ln:create-relation}).
For non-terminal relations, the right hand side of each rule must be transformed (line~\ref{ln:build-rules}) into a linked list of interleaving nodes and symbols as seen in Figure~\ref{fig:ex-relations}.
At this moment, the node set at the start of each rule is initiated with a \emph{new} element, the relation's $node$.

\begin{algorithm}[h]
    \input{algs/backup/get-or-create}
	\caption{Get or create relation.}
	\label{alg:get-or-create}
\end{algorithm}

Algorithm~\ref{alg:process-new} is the core of our approach.
It receives as parameter a new $nodeset$ element, consisting on the $old$ and $new$ sets of nodes, $prev$ and $next$ symbols in the rule it belongs to and it's relation, from the main function and processes the $new$ nodes.
The algorithm behaves in one of two distinct ways, depending on whether the nodeset is at the end of the rule or not.

If the $nodeset$ is in the middle of the rule (lines~\ref{ln:start-advance}-\ref{ln:end-advance}), the procedure advances the derivation.
Instead of simply advancing a dot mark, as it is done by parsers, our approach consults answer nodes for the relation $(a,next.label)$ for each $a \in new$ and passes on those that are not in the $old'$ set of $nodeset'$.

If the $nodeset$ is at the end of it's rule, the procedure updates the relation's set of answers (line~\ref{ln:update-answers}) and notify observers (lines~\ref{ln:start-notify}-\ref{ln:end-notify}).
% (line~\ref{ln:})
% (lines~\ref{ln:}-\ref{ln:})

\begin{algorithm}[h]
    \input{algs/backup/process-new}
	\caption{Process new Nodeset element.}
	\label{alg:process-new}
\end{algorithm}

==> algs/backup/ontologies.tex <==
\begin{table} \centering \begin{tabular}{lrrrr} \hline \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{Query 1} }                                              & \multicolumn{1}{c}{\textbf{Query 1} }   & \multicolumn{1}{c}{\textbf{Query 2} }  & \multicolumn{1}{c}{\textbf{Query 2} }    \\ \textbf{\textbf{Ontology}}  & \multicolumn{1}{l}{\textbf{time(ms)}} & \multicolumn{1}{c}{\textbf{\#results} } & \multicolumn{1}{c}{\textbf{time(ms)} } & \multicolumn{1}{c}{\textbf{\#results} }  \\ \hline
skos & 1 & 810 & 0 & 1 \\ \hline generations & 2 & 2164 & 0 & 0 \\ \hline travel & 3 & 2499 & 0 & 63 \\ \hline univ-bench & 3 & 2540 & 0 & 81 \\ \hline foaf & 4 & 4118 & 0 & 10 \\ \hline people-pets & 9 & 9472 & 0 & 37 \\ \hline funding & 21 & 17634 & 3 & 1158 \\ \hline atom-primitive & 36 & 15454 & 18 & 122 \\ \hline biomedical & 30 & 15156 & 9 & 2871 \\ \hline pizza & 71 & 56195 & 8 & 1262 \\ \hline wine & 72 & 66572 & 1 & 133 \\ \hline 
\end{tabular}
\caption{Performance Evaluation on RDF Databases.}
\label{tab:performance}
\end{table}


==> algs/backup/process-new.tex <==
% \KwIn{$nodeset = (old,new,prev,next,rel)$}
%\KwResult{...}  
\SetKwProg{procedure}{procedure}{}{end}
\procedure{process\_new$(nodeset = (old,new,prev,next,rel))$ }{ %\ciro{(math-like version)}
    $old := old \cup new$ \label{ln:union-old-new} \\ % NÃO coloque esta linha no final
    \If{$next \neq \nil$}{ 
        \ciro{next is a Symbol struct}
        % \tcc{still in the middle of the expression, must advance the derivation}
        $nodeset' := (old',new',next,next',rel)$ \label{ln:start-advance} \ciro{next no lugar de prev' garante que este é o próximo nodeset} \\
        \ForEach{$a \in new$}{     
            $new' := new' \cup get\_or\_create(a,next.label).answers - old'$ 
        }
        \label{ln:end-advance}
   }\Else{
        % \tcc{reached the end of the expression, must update relation's answers and notify observers}
        % \If{$rel$ is \textbf{nested}}{
        %     $new := \set{rel.node}$
        % }
        $rel.answers := rel.answers \cup new$ \label{ln:update-answers} \\
        
        \ForEach{$nodeset' = (old',new',prev',next',rel')$ \observing $rel$}{ \label{ln:start-notify}
            \ForEach{$a \in new$}{     
                $new' := new' \cup get\_or\_create(a,next.label) - old'$
            }
             \label{ln:end-notify}
        }
    }
    $new := \emptyset$ \label{ln:new-empty} % NÃO coloque esta linha no começo
}


==> algs/backup/relogio.tex <==
\section{Experimentos com tempo de relógio}



\begin{table}[htpb]
\centering
\begin{tabular}{@{}llrrrr@{}}
\toprule
\textbf{$G$} & \textbf{$D$} & \textbf{$|V|$} & \textbf{Results} & \textbf{Time} & \textbf{Memory} \\
\midrule

$G_{\ref{gram:same-level}}$ & skos & 43 & 810 & 4 ms & 3.0 Mb \\
$G_{\ref{gram:same-level}}$ & generations & 82 & 2164 & 8 ms & 3.2 Mb \\
$G_{\ref{gram:same-level}}$ & travel & 92 & 2499 & 9 ms & 3.5 Mb \\
$G_{\ref{gram:same-level}}$ & univ\_bench & 90 & 2540 & 14 ms & 3.7 Mb \\
$G_{\ref{gram:same-level}}$ & foaf & 93 & 4118 & 14 ms & 4.1 Mb \\
$G_{\ref{gram:same-level}}$ & people\_pets & 163 & 9472 & 46 ms & 6.9 Mb \\
$G_{\ref{gram:same-level}}$ & funding & 272 & 17634 & 148 ms & 11.8 Mb \\
$G_{\ref{gram:same-level}}$ & atom\_primitive & 142 & 15454 & 193 ms & 14.6 Mb \\
$G_{\ref{gram:same-level}}$ & biomedical & 134 & 15156 & 164 ms & 13.1 Mb \\
$G_{\ref{gram:same-level}}$ & pizza & 359 & 56195 & 414 ms & 18.7 Mb \\
$G_{\ref{gram:same-level}}$ & wine & 468 & 66572 & 410 ms & 21.3 Mb \\
\midrule

$G_{\ref{gram:adjacent-level}}$ & skos & 2 & 1 & 0 ms & 1.6 Mb \\
$G_{\ref{gram:adjacent-level}}$ & generations & 0 & 0 & 0 ms & 1.9 Mb \\
$G_{\ref{gram:adjacent-level}}$ & travel & 32 & 63 & 4 ms & 1.8 Mb \\
$G_{\ref{gram:adjacent-level}}$ & univ\_bench & 42 & 81 & 4 ms & 2.0 Mb \\
$G_{\ref{gram:adjacent-level}}$ & foaf & 13 & 10 & 0 ms & 2.1 Mb \\
$G_{\ref{gram:adjacent-level}}$ & people\_pets & 44 & 37 & 3 ms & 2.5 Mb \\
$G_{\ref{gram:adjacent-level}}$ & funding & 93 & 1158 & 8 ms & 3.2 Mb \\
$G_{\ref{gram:adjacent-level}}$ & atom\_primitive & 124 & 122 & 88 ms & 11.3 Mb \\
$G_{\ref{gram:adjacent-level}}$ & biomedical & 123 & 2871 & 32 ms & 6.4 Mb \\
$G_{\ref{gram:adjacent-level}}$ & pizza & 261 & 1262 & 26 ms & 7.1 Mb \\
$G_{\ref{gram:adjacent-level}}$ & wine & 163 & 133 & 5 ms & 3.5 Mb \\
\midrule

$G_{\ref{gram:bt}}$ & geospecies & 20882 & 226669749 & 637289 ms & 37235.5 Mb \\
\bottomrule
\end{tabular}
\caption{['ontologies-sc\_t-rep-10.tsv', 'ontologies-sc-rep-10.tsv', 'kjp-table6-rep-10.tsv']}
\label{tab:my-table}
\end{table}


\begin{tikzpicture}
    \begin{axis}[
        height=5cm,
        width=7cm,
        grid=major,
        legend pos=north west,
        xlabel=vertices,
        ylabel=Time (ms)
    ]

\addplot coordinates { (0, 0) (50, 43) (100, 325) (150, 936) (200, 1798) (250, 3012) (300, 4449) (350, 7005) (400, 10172) (450, 14566) (500, 17068)};
\addlegendentry{ complete-dense-rep-10.tsv };
\addplot coordinates { (0, 0) (50, 95) (100, 619) (150, 1686) (200, 3217) (250, 6505) (300, 8406) (350, 12653) (400, 18190) (450, 31766) (500, 39054)};
\addlegendentry{ complete-sparse-rep-10.tsv };
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
    \begin{axis}[
        height=5cm,
        width=7cm,
        grid=major,
        legend pos=north west,
        xlabel=vertices,
        ylabel=Memory (MB)
    ]

\addplot coordinates { (0, 1) (50, 4) (100, 10) (150, 18) (200, 22) (250, 39) (300, 45) (350, 53) (400, 61) (450, 134) (500, 103)};
\addlegendentry{ complete-dense-rep-10.tsv };
\addplot coordinates { (0, 1) (50, 6) (100, 14) (150, 24) (200, 31) (250, 52) (300, 66) (350, 80) (400, 94) (450, 218) (500, 174)};
\addlegendentry{ complete-sparse-rep-10.tsv };
\end{axis}
\end{tikzpicture}

\begin{table}[htpb]
\centering
\begin{tabular}{@{}llrrrr@{}}
\toprule
\textbf{Grammar} & \textbf{Graph} & \textbf{$|V|$} & \textbf{Results} & \textbf{Time} & \textbf{Memory} \\
\midrule

an\_bm\_cm\_dn & \Gnk(100,1 & 100 & 5 & 4 ms & 2.4 Mb \\
an\_bm\_cm\_dn & \Gnk(500,1 & 500 & 25 & 10 ms & 4.5 Mb \\
an\_bm\_cm\_dn & \Gnk(2500,1 & 2500 & 161 & 134 ms & 17.0 Mb \\
an\_bm\_cm\_dn & \Gnk(10000,1 & 10000 & 706 & 717 ms & 47.3 Mb \\
an\_bm\_cm\_dn & \Gnk(100,3 & 100 & 56 & 5 ms & 2.7 Mb \\
an\_bm\_cm\_dn & \Gnk(500,3 & 500 & 769 & 44 ms & 7.1 Mb \\
an\_bm\_cm\_dn & \Gnk(2500,3 & 2500 & 3377 & 258 ms & 22.8 Mb \\
an\_bm\_cm\_dn & \Gnk(10000,3 & 10000 & 14583 & 1174 ms & 71.0 Mb \\
an\_bm\_cm\_dn & \Gnk(100,5 & 100 & 312 & 7 ms & 2.7 Mb \\
an\_bm\_cm\_dn & \Gnk(500,5 & 500 & 2207 & 63 ms & 8.0 Mb \\
an\_bm\_cm\_dn & \Gnk(2500,5 & 2500 & 13823 & 450 ms & 28.4 Mb \\
an\_bm\_cm\_dn & \Gnk(10000,5 & 10000 & 77423 & 1874 ms & 103.2 Mb \\
an\_bm\_cm\_dn & \Gnk(100,10 & 100 & 1068 & 18 ms & 3.8 Mb \\
an\_bm\_cm\_dn & \Gnk(500,10 & 500 & 10211 & 264 ms & 15.6 Mb \\
an\_bm\_cm\_dn & \Gnk(2500,10 & 2500 & 102867 & 1769 ms & 65.0 Mb \\
an\_bm\_cm\_dn & \Gnk(10000,10 & 10000 & 784055 & 10291 ms & 349.5 Mb \\
\bottomrule
\end{tabular}
\caption{['kjp-figures23-rep-10.tsv']}
\label{tab:my-table}
\end{table}

\begin{table}[htpb]
\centering
\begin{tabular}{@{}llrrrr@{}}
\toprule
\textbf{Grammar} & \textbf{Graph} & \textbf{$|V|$} & \textbf{Results} & \textbf{Time} & \textbf{Memory} \\
\midrule

sparse & \Gnk(500,1 & 500 & 0 & 8 ms & 3.9 Mb \\
sparse & \Gnk(500,3 & 500 & 19859 & 278 ms & 16.9 Mb \\
sparse & \Gnk(500,5 & 500 & 93114 & 1098 ms & 39.9 Mb \\
sparse & \Gnk(500,10 & 500 & 208715 & 3166 ms & 115.0 Mb \\
\bottomrule
\end{tabular}
\caption{['kjp-table2-rep-10.tsv']}
\label{tab:my-table}
\end{table}

\begin{table}[htpb]
\centering
\begin{tabular}{@{}llrrrr@{}}
\toprule
\textbf{Grammar} & \textbf{Graph} & \textbf{$|V|$} & \textbf{Results} & \textbf{Time} & \textbf{Memory} \\
\midrule

sl & \Gnk(100,5 & 88 & 360 & 4 ms & 2.3 Mb \\
sr & \Gnk(100,5 & 88 & 360 & 4 ms & 2.3 Mb \\
\bottomrule
\end{tabular}
\caption{['kjp-table3-rep-10.tsv']}
\label{tab:my-table}
\end{table}

\begin{table}[htpb]
\centering
\begin{tabular}{@{}llrrrr@{}}
\toprule
\textbf{Grammar} & \textbf{Graph} & \textbf{$|V|$} & \textbf{Results} & \textbf{Time} & \textbf{Memory} \\
\midrule

ambiguous & \Gnk(100,5 & 100 & 1904 & 11 ms & 3.5 Mb \\
\bottomrule
\end{tabular}
\caption{['kjp-table4-rep-10.tsv']}
\label{tab:my-table}
\end{table}


\begin{tikzpicture}
    \begin{axis}[
        height=5cm,
        width=7cm,
        grid=major,
        legend pos=north west,
        xlabel=vertices,
        ylabel=Time (ms)
    ]

\addplot coordinates { (0, 0) (50, 258) (100, 2356) (150, 7277) (200, 18273) (250, 45277) (300, 56458) (350, 101906) (400, 169101) (450, 371072) (500, 475549)};
\addlegendentry{ complete-ab\_ambiguous-rep-10.tsv };
\addplot coordinates { (0, 0) (50, 345) (100, 3401) (150, 12342) (200, 36652) (250, 58179) (300, 122685) (350, 254971) (400, 388571) (450, 444283) (500, 638964)};
\addlegendentry{ complete-ab\_unambiguous-rep-10.tsv };
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
    \begin{axis}[
        height=5cm,
        width=7cm,
        grid=major,
        legend pos=north west,
        xlabel=vertices,
        ylabel=Memory (MB)
    ]

\addplot coordinates { (0, 1) (50, 6) (100, 15) (150, 26) (200, 33) (250, 57) (300, 69) (350, 85) (400, 101) (450, 221) (500, 177)};
\addlegendentry{ complete-ab\_ambiguous-rep-10.tsv };
\addplot coordinates { (0, 1) (50, 7) (100, 16) (150, 23) (200, 30) (250, 52) (300, 64) (350, 79) (400, 91) (450, 200) (500, 162)};
\addlegendentry{ complete-ab\_unambiguous-rep-10.tsv };
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
    \begin{axis}[
        height=5cm,
        width=7cm,
        grid=major,
        legend pos=north west,
        xlabel=vertices,
        ylabel=Time (ms)
    ]

\addplot coordinates { (0, 0) (50, 1) (100, 5) (150, 9) (200, 8) (250, 8) (300, 11) (350, 16) (400, 24) (450, 42) (500, 44)};
\addlegendentry{ string-ab\_ambiguous-rep-10.tsv };
\addplot coordinates { (0, 0) (50, 1) (100, 3) (150, 4) (200, 4) (250, 4) (300, 8) (350, 10) (400, 12) (450, 16) (500, 20)};
\addlegendentry{ string-ab\_unambiguous-rep-10.tsv };
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
    \begin{axis}[
        height=5cm,
        width=7cm,
        grid=major,
        legend pos=north west,
        xlabel=vertices,
        ylabel=Memory (MB)
    ]

\addplot coordinates { (0, 1) (50, 1) (100, 2) (150, 3) (200, 3) (250, 3) (300, 4) (350, 4) (400, 4) (450, 7) (500, 7)};
\addlegendentry{ string-ab\_ambiguous-rep-10.tsv };
\addplot coordinates { (0, 1) (50, 1) (100, 2) (150, 2) (200, 2) (250, 3) (300, 3) (350, 3) (400, 4) (450, 4) (500, 5)};
\addlegendentry{ string-ab\_unambiguous-rep-10.tsv };
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
    \begin{axis}[
        height=5cm,
        width=7cm,
        grid=major,
        legend pos=north west,
        xlabel=vertices,
        ylabel=Time (ms)
    ]

\addplot coordinates { (0, 0) (50, 38) (100, 238) (150, 794) (200, 1527) (250, 2626) (300, 4004) (350, 5678) (400, 7669) (450, 12180) (500, 14975)};
\addlegendentry{ cycle-dense-rep-10.tsv };
\addplot coordinates { (0, 0) (50, 18) (100, 100) (150, 282) (200, 485) (250, 802) (300, 1037) (350, 1356) (400, 1664) (450, 2433) (500, 2883)};
\addlegendentry{ cycle-sparse-rep-10.tsv };
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
    \begin{axis}[
        height=5cm,
        width=7cm,
        grid=major,
        legend pos=north west,
        xlabel=vertices,
        ylabel=Memory (MB)
    ]

\addplot coordinates { (0, 1) (50, 4) (100, 8) (150, 15) (200, 18) (250, 27) (300, 32) (350, 37) (400, 42) (450, 90) (500, 73)};
\addlegendentry{ cycle-dense-rep-10.tsv };
\addplot coordinates { (0, 1) (50, 4) (100, 8) (150, 14) (200, 19) (250, 30) (300, 38) (350, 43) (400, 49) (450, 85) (500, 82)};
\addlegendentry{ cycle-sparse-rep-10.tsv };
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
    \begin{axis}[
        height=5cm,
        width=7cm,
        grid=major,
        legend pos=north west,
        xlabel=vertices,
        ylabel=Time (ms)
    ]

\addplot coordinates { (0, 0) (50, 11) (100, 66) (150, 224) (200, 439) (250, 787) (300, 1170) (350, 1633) (400, 2134) (450, 2842) (500, 3551)};
\addlegendentry{ path-dense-rep-10.tsv };
\addplot coordinates { (0, 0) (50, 11) (100, 35) (150, 131) (200, 263) (250, 422) (300, 592) (350, 820) (400, 961) (450, 1254) (500, 1511)};
\addlegendentry{ path-sparse-rep-10.tsv };
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
    \begin{axis}[
        height=5cm,
        width=7cm,
        grid=major,
        legend pos=north west,
        xlabel=vertices,
        ylabel=Memory (MB)
    ]

\addplot coordinates { (0, 1) (50, 2) (100, 5) (150, 10) (200, 13) (250, 17) (300, 21) (350, 26) (400, 28) (450, 34) (500, 44)};
\addlegendentry{ path-dense-rep-10.tsv };
\addplot coordinates { (0, 1) (50, 3) (100, 6) (150, 11) (200, 15) (250, 19) (300, 25) (350, 30) (400, 35) (450, 43) (500, 50)};
\addlegendentry{ path-sparse-rep-10.tsv };
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
    \begin{axis}[
        height=5cm,
        width=7cm,
        grid=major,
        legend pos=north west,
        xlabel=vertices,
        ylabel=Time (ms)
    ]

\addplot coordinates { (0, 0) (50, 43) (100, 325) (150, 936) (200, 1798) (250, 3012) (300, 4449) (350, 7005) (400, 10172) (450, 14566) (500, 17068)};
\addlegendentry{ complete-dense-rep-10.tsv };
\addplot coordinates { (0, 0) (50, 95) (100, 619) (150, 1686) (200, 3217) (250, 6505) (300, 8406) (350, 12653) (400, 18190) (450, 31766) (500, 39054)};
\addlegendentry{ complete-sparse-rep-10.tsv };
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
    \begin{axis}[
        height=5cm,
        width=7cm,
        grid=major,
        legend pos=north west,
        xlabel=vertices,
        ylabel=Memory (MB)
    ]

\addplot coordinates { (0, 1) (50, 4) (100, 10) (150, 18) (200, 22) (250, 39) (300, 45) (350, 53) (400, 61) (450, 134) (500, 103)};
\addlegendentry{ complete-dense-rep-10.tsv };
\addplot coordinates { (0, 1) (50, 6) (100, 14) (150, 24) (200, 31) (250, 52) (300, 66) (350, 80) (400, 94) (450, 218) (500, 174)};
\addlegendentry{ complete-sparse-rep-10.tsv };
\end{axis}
\end{tikzpicture}


==> algs/backup/starter.tex <==
\KwIn{$G = (\nonterminals,\terminals,\rules), ~Q \subseteq V \times \nonterminals, ~D \subseteq V\times E \times V $}

\KwResult{$Res:V\times\nonterminals \mapsto V$}  
\SetKwProg{procedure}{procedure}{}{end}
\procedure{eval}{
    $Res:V\times \nonterminals \mapsto V$
    
    $Dep:V\times \nonterminals \mapsto Ids^2$
    
    $I : ...$
    
    \While{$\exists v\u \in C, $}{
        mark(v)
        
        \If{$\Rule{S}{... ~\set{v\u, ...} ~t ~C'}$}{
            \ForEach{$v' s.t. (v,t,v') \in D$}{
                $C' := C' ~\munion~ \set{v' {\u}}$
            }
        }\ElseIf{$\Rule{S}{... ~\set{v\u, ...} ~A ~C'}$}{
            \ForEach{$\Rule{A}{\alpha_1 ~...~ \alpha_n} \in \rules$}{
                \If{$\Rule{A}{C_0 ~\alpha_1 ~C_1 ~... ~\alpha_n ~C_n} \notin I$}{
                    $I := I ~\munion~ \set{\Rule{A}{\set{v} ~\alpha_1 ~\set{} ~... ~\alpha_n ~\set{}}}$
                }\Else{
                    $C' := C' ~\munion~ \set{v'{\u} ~|~ v' \in Res(v,A)} $
                }
                $Dep(v,A) := Dep(v,A) \cup C'$
            }
        }\ElseIf{$\Rule{A}{\set{a}~...~C_n=\set{v, ...}} \in I$}{
            $Res(a,A) := Res(a,A) \cup \set{v}$
            
            \ForEach{$C \in Dep(a,A)$}{
                $C := C ~\munion~ \set{v\u}$
            }
        }
        
    }
    \Return Res
}


==> fig/ex-relations.tex <==
\begin{tikzpicture}[minimum width=0.5cm, minimum height = 0.5cm]

\node[anchor=west] at (-1,0.5) {\textbf{(A)} $\Rule{S}{(~ S ~) ~ }$};
% \node[anchor=west] at (-1,0.5) {\textbf{(A)} $\Rule{S}{\set{a} ~ ( ~ \set{b,c^*,d^*} ~ S ~ \set{b} ~ ) ~ \set{e}}$};


\Nodeset{start}{0}{0}{a}{}
\Symbol{1}{0}{open}{(}
\Nodeset{n2}{2}{0}{b}{c,d}
\Symbol{3}{0}{S}{S}
\Nodeset{n3}{4}{0}{b}{}
\Symbol{5}{0}{close}{)}
\Nodeset{end}{6}{0}{e}{}

\draw[->, >=stealth] (start-0) to (open);
\draw[->, >=stealth] (open) to (n2-2);
\draw[->, >=stealth] (n2-0) to (S);
\draw[->, >=stealth] (S) to (n3-2);
\draw[->, >=stealth] (n3-0) to (close);
\draw[->, >=stealth] (close) to (end-2);

\node[anchor=west] at (-1,-2) {\textbf{(B)} $\Rule{S}{\epsilon}$};
% \node[anchor=west] at (-1,-2) {\textbf{(B)} $\Rule{S}{ \set{a}}$};
\Nodeset{a2}{0}{-2.5}{a}{}

\node[anchor=west] at (-1,-4.5) {\textbf{(C)} $\R{a}{S} = \set{a,e}$};

\end{tikzpicture}

==> fig/transitions.tex <==
\begin{tikzpicture}[minimum width=0.6cm, minimum height = 0.5cm]
\node[anchor=west] at (0,0) {\textbf{(A)} $\Rule{S}{\set{v\u}}$};

\Nodeset{n}{1}{-0.5}{v\u}

%\node[above right = 2cm and 3cm of a] (e) {e};
\node[right = of n-0] (leadsto) {$\leadsto$};

\Nodeset{n}{1}{-0.5}{v\u}

\end{tikzpicture}


\smallskip


\begin{tikzpicture}[minimum width=0.6cm, minimum height = 0.5cm]
\node[anchor=west] at (0,0) {\textbf{(B)} $\Rule{S}{(~ S ~) ~ }$};
\end{tikzpicture}


\smallskip


\begin{tikzpicture}[minimum width=0.6cm, minimum height = 0.5cm]
\node[anchor=west] at (0,0) {\textbf{(C)} $\Rule{S}{(~ S ~) ~ }$};
% \node[anchor=west] at (-1,0.5) {\textbf{(A)} $\Rule{S}{\set{a} ~ ( ~ \set{b,c^*,d^*} ~ S ~ \set{b} ~ ) ~ \set{e}}$};
\Nodeset{a2}{1}{-0.5}{a}{}
\end{tikzpicture}

\smallskip

\begin{tikzpicture}[minimum width=0.6cm, minimum height = 0.5cm]
\node[anchor=west] at (0,0) {\textbf{(D)} $\R{a}{S} = \set{a,e}$};
\Nodeset{start}{0}{0}{a}
\Symbol{1}{0}{open}{(}
\Nodeset{n2}{2}{0}{b,c,d}
\Symbol{3}{0}{S}{S}
\Nodeset{n3}{4}{0}{b}
\Symbol{5}{0}{close}{)}
\Nodeset{end}{6}{0}{e}

\draw[->, >=stealth] (start-0) to (open);
\draw[->, >=stealth] (open) to (n2-0);
\draw[->, >=stealth] (n2-0) to (S);
\draw[->, >=stealth] (S) to (n3-0);
\draw[->, >=stealth] (n3-0) to (close);
\draw[->, >=stealth] (close) to (end-0);
\end{tikzpicture}

==> tables/kjp-ambiguous.tex <==
\centering\small
\begin{tabular}{@{}lrr|rr|rr@{}}
\toprule
&&& \multicolumn{2}{c|}{\textbf{TI-based}} & \multicolumn{2}{c}{\textbf{LL}~\cite{comlan}} \\
\textbf{Grammar \& Graph} & \textbf{$|V|$} & \textbf{Results} & \textbf{Time} & \textbf{Memory} & \textbf{Time} & \textbf{Memory}\\
\midrule

$G_{\ref{gram:kjp_ambiguous}}$, \Gnk(100,5) & 100 & 1904 & 15 ms & 3.5 Mb & 3314 ms & 7.2 Mb \\
\bottomrule
\end{tabular}

==> tables/kjp-sl-sr.tex <==
\begin{tabular}{@{}lrr|rr|rr@{}}
\toprule
&&& \multicolumn{2}{c|}{\textbf{This work}} & \multicolumn{2}{c}{\textbf{LL}~\cite{comlan}} \\
\textbf{Grammar \& Graph} & \textbf{$|V|$} & \textbf{Results} & \textbf{Time} & \textbf{Memory} & \textbf{Time} & \textbf{Memory}\\
\midrule


$G_{\ref{gram:kjp_sl}}$, \Gnk(100,5) & 88 & 360 & 4 ms & 2.6 Mb \\
$G_{\ref{gram:kjp_sr}}$, \Gnk(100,5) & 88 & 360 & 4 ms & 2.3 Mb \\
\bottomrule
\end{tabular}

==> tables/kjp-sparse.tex <==
\begin{tabular}{@{}lrr|rr|rr@{}}
\toprule
&&& \multicolumn{2}{c|}{\textbf{This work}} & \multicolumn{2}{c}{\textbf{LL}~\cite{comlan}} \\
\textbf{Grammar \& Graph} & \textbf{$|V|$} & \textbf{Results} & \textbf{Time} & \textbf{Memory} & \textbf{Time} & \textbf{Memory}\\
\midrule

$G_{\ref{gram:kjp_sparse}}$, \Gnk(500,1 & 500 & 0 & 8 ms & 3.9 Mb & 6 ms & 7.5 Mb \\
$G_{\ref{gram:kjp_sparse}}$, \Gnk(500,3 & 500 & 19859 & 274 ms & 17.3 Mb & 264947 ms & 17.5 Mb \\
$G_{\ref{gram:kjp_sparse}}$, \Gnk(500,5 & 500 & 93114 & 1125 ms & 39.8 Mb \\
$G_{\ref{gram:kjp_sparse}}$, \Gnk(500,10 & 500 & 208715 & 3264 ms & 113.8 Mb \\
\bottomrule
\end{tabular}
